Stabilization of singularly perturbed networked control systems over a single channel

This paper studies the emulation-based stabilization of nonlinear networked control systems with two time scales. We address the challenge of using a single communication channel for transmitting both fast and slow variables between the plant and the controller. A novel dual clock mechanism is proposed to schedule transmissions for this purpose. The system is modeled as a hybrid singularly perturbed dynamical system, and singular perturbation analysis is employed to determine individual maximum allowable transmission intervals for both fast and slow variables, ensuring semi-global practical asymptotic stability. Enhanced stability guarantees are also provided under stronger assumptions. The efficacy of the proposed method is illustrated through a numerical example.

==> Chapters/4.5_Stefan_s_Clock_Mechanism.tex <==
\aim{
It is noteworthy that \cite[Section 4.5.1]{Stefan_thesis} proposed a natural approach to extend from the two-channel case to the single-channel case, which is to keep the same two-channel clock variables. That is, the timer in \cite{Stefan_thesis} satisfies
%
\begin{subequations}
    \begin{align}
    &\tau_{\text{miati}}^s \leq t_{k+1}^s - t_k^s \leq \tau_{\text{mati}}^s, \forall t_k^s,t_{k+1}^s\in \mathcal{T}^s, k\in\mathbb{Z}_{\geq 0}, 
    \\
    &\tau_{\text{miati}} \leq t_{j+1}^f - t_j^f \leq \tau_{\text{mati}}^f ,  \forall t_j^f, t_{j+1}^f  \in \mathcal{T}^f, j \in\mathbb{Z}_{\geq 0}, 
    \\
    &\tau_{\text{miati}} \leq t_{\ell+1} - t_\ell, \quad \qquad \ \forall t_\ell, t_{\ell + 1} \in \mathcal{T}, \ell \in \mathbb{Z}_{\geq 0}, \label{eqn: Stefan miati}
    \end{align}
    \label{eqn: Stefan timer}
\end{subequations}
where $\tau_{\text{mati}}^f$ denotes the MATI between two consecutive fast updates, and $\tau_{\text{miati}}$ and $\tau_{\text{mati}}^s$ are defined in the same manner as in (\ref{eqn: New Timer}). We emphasize that $\tau_{\text{miati}}^s$ in \eqref{eqn: Stefan timer} is added here to avoid Zeno solutions when $\epsilon\to 0$, an issue that was not reported in \cite{Stefan_thesis}, since the authors did not study stability for the single-channel case with the timer \eqref{eqn: Stefan timer}.
%
Moreover, it was reported in \cite{Stefan_thesis}, that in order to obtain a feasible sequence of transmission times for the clock formulation in \eqref{eqn: Stefan timer}, then $\tau_{\text{miati}} \leq  \tfrac{1}{2}\tau_{\text{mati}}^f$ must hold.
Compared to the findings in \cite{Stefan_thesis}, \aim{the clock mechanism \eqref{eqn: New Timer} can stabilize the system with less bandwidth, this will be shown later.}

\begin{figure}[H]
    \centering
    \includegraphics[width = \linewidth]{Figures/Stefan Clock Mechanism Illustration.pdf}
    \caption{Flow set and jump set}
    \label{fig: Stefan timer}
\end{figure} \todo[inline]{Change the name of sets}

Before we present our NCS in hybrid system, we first need to define the timers correspond to the clock mechanism \eqref{eqn: Stefan timer}. We will keep using $\tau_s$ to describe the inter-transmission time between any two consecutive slow transmissions, as previously defined in $\mathcal{H}_1$. 
%
To streamline our discussion and avoid redundancy in restating all the Assumptions and Lemma, in this section, we will redefine the parameter $\tau$ as the time elapsed since the most recent fast transmission.
%
Consequently, the single-channel SPNCS, which incorporates the clock mechanism defined in equation \eqref{eqn: Stefan timer}, can be depicted as a hybrid system denoted as $\mathcal{H}_3$, which we describe below.






\begin{equation*}
    \mathcal{H}_3:\left\{
\begin{aligned}
    \dot{\xi} &= F(\xi, \cyan{\epsilon}),\ \xi \in \mathcal{C}_3^\epsilon, \\
    \xi^+ &\in G_3(\xi), \ \xi\in \mathcal{D}_{3,s}^\epsilon \cup \mathcal{D}_{3,f}^\epsilon,
\end{aligned}
    \right.
\end{equation*}
where 
\begin{align*}
    G_3(\xi) \coloneqq \left\{ 
    \begin{aligned}
    &G_{3,s}(\xi), && \xi\in\mathcal{D}_{3,s}^\epsilon \setminus \mathcal{D}_{3,f}^\epsilon , \\
    &G_f(\xi), && \xi\in\mathcal{D}_{3,f}^\epsilon \setminus \mathcal{D}_{3,s}^\epsilon ,\\
    &\{G_{3,s}(\xi),G_f(\xi)\},&& \xi\in \mathcal{D}_{3,s}^\epsilon\cap\mathcal{D}_{3,f}^\epsilon ,
    \end{aligned}
    \right.  
    \end{align*}
and $F$ and $G_f$ come from $\mathcal{H}_1$. The flow map $G_{3,s}$ is defined such that $G_{3,s} \coloneqq (x, h_s(\kappa_s, e_s), 0, \kappa_s +1, z, e_f, \tau, \kappa_f)$.

The jump and flow sets are defined as 
\begin{align*}
    \mathcal{D}_{3,s}^\epsilon \coloneqq & \left\{\xi \in \mathbb{X} \; | \; \tau_s \in [\tau_{\text{miati}}^s, \tau_{\text{mati}}^s] \right. \\
    & \qquad \qquad  \qquad \qquad  \wedge \epsilon \tau \in  [\tau_{\text{miati}}, \tau_{\text{mati}}^f - \tau_{\text{miati}}]  \},
    \\
    \mathcal{D}_{3,f}^\epsilon \coloneqq &\left\{\xi \in \mathbb{X} \; | \; \tau_s \in [\tau_{\text{miati}}, \tau_{\text{mati}}^s-\tau_{\text{miati}}] \right. \\
    & \qquad \qquad \qquad \qquad \quad  \wedge\; \epsilon \tau \in  [\tau_{\text{miati}}, \tau_{\text{mati}}^f]  \},
    \\
    \mathcal{C}_3^\epsilon \coloneqq & 
        \mathcal{D}_{3,s}^\epsilon \cup \mathcal{D}_{3,f}^\epsilon \cup \mathcal{C}_{3,a}^\epsilon \cup \mathcal{C}_{3,b}^\epsilon  
\end{align*}
with $\mathcal{C}_{3,a}^\epsilon \coloneqq \{ \xi \in \mathbb{X} \ | \ \tau_s \in [0, \tau_{\text{miati}}]  \wedge \epsilon \tau \in [0,\tau_s + ( \tau_{\text{mati}}^f - \tau_{\text{miati}})] \} $ and 
$\mathcal{C}_{3,b}^\epsilon \coloneqq \{ \xi \in \mathbb{X} \;|\; \tau_s \in [\tau_{\text{miati}}, \epsilon \tau + (\tau_{\text{mati}}^s - \tau_{\text{miati}})]  \wedge \epsilon \tau \in  [0, \tau_{\text{miati}}]  \}$. 
We emphasize again that $\tau$ denotes the time elapsed since the last fast transmission.


The stability result of $\mathcal{H}_3$ is formalized in Corollary \ref{Corollary Stefan Timer} below, and its proof follows similar steps as the proof of Theorem \ref{Theorem H_1}. To achieve this, we need to first define a ``patched" system for $\mathcal{H}_3$, namely, $\mathcal{H}_4$, where the patch is depicted by the red region in Figure \ref{fig: Stefan timer}. Then we changing the coordinate from $z$ to $y$ and write $\tau_{\text{mati}}^f = \epsilon T^* $ and $\tau_{\text{miati}} = \epsilon aT^*$, $a \in (0,1)$, we get $\mathcal{H}_4^y$. 

\begin{equation}
    \mathcal{H}_4^y:\left\{
\begin{aligned}
    \dot{\xi}^y &= F^y(\xi^y, \cyan{\epsilon}),\ \xi^y \in \mathcal{C}_4^{y,\epsilon}, \\
    {\xi^y}^+ &\in G_4^y(\xi^y), \ \xi^y\in \mathcal{D}_{4,s}^{y,\epsilon} \cup \mathcal{D}_{4,f}^{y,\epsilon},
\end{aligned}
    \right.
    \label{eqn: H_4^y}
\end{equation}
where $\mathcal{D}_{4,s}^{y,\epsilon} = \{\xi^y \in \mathbb{X} | \tau_s \in [ \tau_{\text{miati}}^s, \tau_{\text{mati}}^s \wedge \tau \in [aT^*, (1-a)T^*] \}$, $\mathcal{D}_{4,f}^{y,\epsilon} = \mathcal{D}_f^{y,\epsilon}$,  $\mathcal{C}_4^{y,\epsilon}\coloneqq \mathcal{D}_{4,s}^{y,\epsilon} \cup \mathcal{D}_{4,f}^{y,\epsilon} \cup \{ \xi^y \in \mathbb{X} | \tau_s \in [0, \epsilon T^*] \wedge \tau \in [0, T^*]\} \cup  \{ \xi^y \in \mathbb{X} | \tau_s \in [0, \tau_{\text{mati}}^s \wedge \tau \in [0, aT^*]\} $.

Additionally, we have
\begin{align*}
    G_4^y(\xi^y) \coloneqq \left\{ 
    \begin{aligned}
    &G_{4,s}^y(\xi^y),  \;\xi^y\in\mathcal{D}_{4,s}^{y,\epsilon} \setminus \mathcal{D}_{4,f}^{y,\epsilon} , \\
    &G_f^y(\xi^y),  \;  \xi^y \in\mathcal{D}_{4,f}^{y,\epsilon} \setminus \mathcal{D}_{4,s}^{y,\epsilon} ,\\
    &\{G_{4,s}^y(\xi^y),G_f^y(\xi^y)\}, \; \xi^y\in \mathcal{D}_{4,s}^{y,\epsilon} \cap \mathcal{D}_{4,f}^{y,\epsilon},
    \end{aligned}
    \right. 
\end{align*}
where $G_{4,s}^y(\xi_y) \coloneqq \big(x, h_s(\kappa_s, e_s), 0, \kappa_s + 1, \red{h_y(x,e_s,y)},  e_f,$ $ \tau, \kappa_f \big)$. 





Subsequently, we can obtain the boundary-layer system and reduced system for the $\mathcal{H}_4^y$. We note that the boundary-layer and reduced system derived from $\mathcal{H}_2^y$ will coincide with those obtained from the $\mathcal{H}_4^y$, therefore, we will keep using $\mathcal{H}_r$ and $\mathcal{H}_{bl}$ to denote the reduced and boundary-layer system of $\mathcal{H}_4$. Consequently, Lemma \ref{Lemma MATI} applies to the boundary-layer and reduced system of $\mathcal{H}_4$.
%
\begin{corollary}
Considering system $\mathcal{H}_3$ and suppose Assumption \ref{Assumption reduced model} and \ref{Assumption boundary layer system} hold, and Assumption \ref{Assumption interconnection} hold for almost all $\xi^y \in \mathcal{C}_4^{y,\epsilon}$.
%
%Let $b_1$, $b_2$, and $b_3$ come from Assumption \ref{Assumption interconnection} and $a_1$ and $a_2$ come from Lemma \ref{Lemma MATI}.
%%%%%%%%%%%%%%%%%%%%%%%%
\cyan{Let $L_s$ and $\gamma_s$ come from Assumption \ref{Assumption reduced model}, and $L_f$ and $\gamma_f$ come from Assumption \ref{Assumption boundary layer system}.
Let $b_1$, $b_2$, and $b_3$ come from Assumption \ref{Assumption interconnection} and $a_1$, $a_2$, \cyan{$\lambda_s^*$} and \cyan{$\lambda_f^*$} come from Lemma \ref{Lemma MATI}.
}
%%%%%%%%%%%%%%%%%%%%%%
Then\sout{, for any $\lambda_s^* \in (\lambda_s,1)$ and $\lambda_f^* \in (\lambda_f, 1)$,} there exists $\epsilon^*  = \tfrac{a_1 a_2}{a_1 b_3 + b_1 b_2}$ such that for all $0<\epsilon<\epsilon^*$, $\tau_{\text{mati}}^s \leq T(L_s, \gamma_s, \lambda_s^*)$ and $\tau_{\text{mati}}^f \leq \epsilon T(L_f, \gamma_f,\lambda_f^*)$, the set $\mathcal{E}$ is UGAS for system $\mathcal{H}_3$. 
\label{Corollary Stefan Timer}
\end{corollary}
\todo{Wrong!!! not UGAS}
\begin{proof}
    The proof of Corollary \ref{Corollary Stefan Timer} is shown in the Appendix.
\end{proof}


\begin{corollary}
Considering system $\mathcal{H}_3$ and suppose the conditions in Corollary \ref{Corollary Stefan Timer} hold, additionally, Assumption \ref{Assumption Exponential} holds. Let $b_1$, $b_2$, and $b_3$ come from Assumption \ref{Assumption interconnection} and $a_1$ and $a_2$ come from Lemma \ref{Lemma MATI}. Then there exist $\epsilon^* = \tfrac{a_1 a_2}{a_1 b_3 + b_1 b_2} $ such that for all $0<\epsilon<\epsilon^*$, $\tau_{\text{mati}}^s \leq T(L_s, \gamma_s, \lambda_s^*)$ and $\tau_{\text{mati}} \leq \epsilon T(L_f, \gamma_f,\lambda_f^*)$, the following statement holds:

There exists a $\tau_{\text{miati}}^{s,*} > 0$, such that if $\tau_{\text{miati}}^{s,*} \red{<} \tau_{\text{mati}}^s - \tau_{\text{miati}}$, $\mathcal{H}_3$ is UGES w.r.t $\mathcal{E}$.
\label{Corollary Stefan Exponential decay}
\end{corollary}
\begin{proof}
    The proof is similar to Corollary \ref{Corollary Exponential decay}.
\end{proof}
}
\begin{remark}
\aim{
In analytical terms, for the plant and controller pair, the upper bound of $\tau_{\text{mati}}$ in (\ref{eqn: New Timer}) that guarantees UGAS (UGES) for $\mathcal{H}_1$ will have the same value as $\tau_{\text{mati}}^f$ in (\ref{eqn: Stefan timer}) that guarantees UGAS (UGES) for $\mathcal{H}_3$. 
However, the clock (\ref{eqn: Stefan timer}) imposes the condition that $\tau_{\text{miati}} \leq \tfrac{1}{2}\tau_{\text{mati}}^f$ , whereas (\ref{eqn: New Timer}) only requires that $\tau_{\text{miati}} \leq \tau_{\text{mati}}$. Consequently, in order to achieve an analytical guarantee of stability, (\ref{eqn: Stefan timer}) requires approximately twice the bandwidth of (\ref{eqn: New Timer}).}

In practical terms, the feasibility condition $\tau_{\text{miati}} \leq  \tfrac{1}{2}\tau_{\text{mati}}^f$ may force the system to wait longer to transmit, which can lead to instability. This is demonstrated in the following. Consider the example from \cite[Section 4.4]{Stefan_thesis}, where the same plant and controller are used, but the slow and fast states are transmitted via one channel. 
Let $\tau_{\text{miati}}^*$ be the smallest MIATI the channel can provide, and suppose $\tau_{\text{miati}}^*=30.4ms$. Then, clocks (\ref{eqn: New Timer}) and (\ref{eqn: Stefan timer}) are feasible if and only if $\tau_{\text{mati}} \geq \tau_{\text{miati}}^*$ and $\tau_{\text{mati}}^f \geq 2\tau_{\text{miati}}^*$, respectively. We select $\tau_{\text{mati}} = 30.4ms$ and $ \tau_{\text{mati}}^f = 60.8ms$. 
%
To simulate the worst-case scenario, we set the priority to flow. 
Fig. \ref{fig: comparison-example} shows the system trajectories with clock (\ref{eqn: New Timer}) and (\ref{eqn: Stefan timer}), respectively. 
%
It is evident that the system cannot be guaranteed to be stable with the use of the smallest feasible value of $\tau_{\text{mati}}^f$ in clock proposed in (\ref{eqn: Stefan timer}). 
%
In contrast, clock proposed in (\ref{eqn: New Timer}) can stabilize the system with a feasible $\tau_{\text{mati}}$.
\end{remark}
%
\begin{figure}[ht]
    \centering
    \hfill
    \begin{minipage}[t]{0.49\linewidth}
    \centering
    % \includegraphics[width = \linewidth]{Figures/Stable example.pdf}
    \includegraphics[width = \linewidth]{Figures/Weixuan_timer.eps}
    \end{minipage}
    \begin{minipage}[t]{0.49\linewidth}
     % \includegraphics[width = \linewidth]{Figures/Unstable example.pdf}
       \includegraphics[width = \linewidth]{Figures/Stefan_timer.eps}
    \end{minipage}
    \caption{(Left) Batch reactor with clock (\ref{eqn: New Timer}); (Right) Batch reactor with clock (\ref{eqn: Stefan timer}).}
     \label{fig: comparison-example}
\end{figure}


% \aim{
% \subsection{Two Channel Case}
% Suppose for that same plant and controller pain, we now have two channels and each is dedicated to transmit slow and fast signal, respectively. Then the component \eqref{eqn: Stefan miati} and the requirement of $\tau_{\text{miati}} \leq \tau_{\text{mati}}^f$ in clock mechanism \eqref{eqn: Stefan timer} are no longer required.



% }



\cyan{
\begin{remark}
    We note that \cite{SPNCS} study a two-channel SPNCS with different plant and controller configurations, and our results are also applicable to the SPNCS in \cite{SPNCS} when only one channel is available.
\end{remark}
}


==> Chapters/7.5_Stable_subsystem_Slow.tex <==
\subsection{Stable slow subsystem}
The second scenario is when the plant has a stable slow subsystem. A controller is designed to stabilise the fast subsystem.
Subsequently, the plant only needs to transmit fast output $y_f$ and the controller only has fast control input $u_f$. 
The plant and controller shown below are in the form of \eqref{eqn:plant} and \eqref{eqn:controller}, where $k_{ps} $ and $k_{cs}$ are removed.
\begin{equation*}
    \mathcal{P}\!:\!
    \begin{cases}
    \dot x_p \!\!\!\!\!\!&= f_p(x_p, z_p,\hat u)\\
    \epsilon \dot z_p\!\!\!\!\!\! &= g_p(x_p, z_p, \hat u) \\
    y_p \!\!\!\!\!\!&= y_f = k_{p_f}(x_p,z_p)  , 
    \end{cases} \;
    \mathcal{C}\!:\!
    \begin{cases}
    \dot x_c \!\!\!\!\!\!&= f_c(x_c, z_c, \hat{y}_p)\\
    \epsilon \dot z_c \!\!\!\!\!\!&= g_c(x_c, z_c, \hat y_p) \\
    u \!\!\!\!\!\!&= u_f = k_{c_f}(x_c,z_c) ,
    \end{cases}
\end{equation*}

Given the exclusive presence of fast transmissions within the communication channel, a simpler version of clock mechanism \eqref{eqn: Stefan timer} is used to govern the system dynamics as follows:
\begin{equation*}
    \tau_{\text{miati}}^f \leq t_{k+1}^f - t_k^f \leq \tau_{\text{mati}}^f, \ \forall t_k^f, t_{k+1}^f\in \mathcal{T}^f, k \in \mathbb{Z}_{\geq 0},
\end{equation*}
where $\tau_{\text{miati}}^f \geq \tau_{\text{miati}}^f$. Moreover, the networked induced error is $e_f =  (\hat{y}_f - y_f, \hat{u}_f - u_f)$ and $e_s$ does not exist. By define the state $\xi_6 \coloneqq (x,z,e_f, \tau_f, \kappa_f,)\in \mathbb{X}_6$, where $\mathbb{X}_6\coloneqq \mathbb{R}^{n_x} \times \mathbb{R}^{n_z} \times \mathbb{R}^{n_{e_f}}\times  \mathbb{R}_{\geq 0} \times \mathbb{Z}_{\geq 1} $, we can define our system by the hybrid model $\mathcal{H}_6$, which we skip its expression here.


% \begin{equation*}
%     \mathcal{H}_5:\left\{
% \begin{aligned}
%     \dot{\xi}_5 &= F_5(\xi_5),\ \xi_5 \in \mathcal{C}_5, \\
%     \xi^+ &= G_{5,s}(\xi_5), \ \xi_5 \in \mathcal{D}_{5,s},
% \end{aligned}
%     \right.
% \end{equation*}
% where $F_5(\xi_5) \coloneqq \big(f_x(x,z,e_s,e_f), f_{e_s}(x,z,e_s,e_f),1,0,$ $\tfrac{1}{\epsilon} g_z(x,z,e_s,e_f) \big)$, $C_5 \coloneqq \{ \xi_5 \in \mathbb{X}_5 | \tau_s \in [0, \tau_{\text{mati}}^s]\}$ , $G_{5,s}(\xi_5) \coloneqq (x, h_s(\kappa_s, e_s), 0, \kappa_s + 1, z)$ and $D_{5,s} \coloneqq \{ \xi_5 \in \mathbb{X}_5 | \tau_s \in [\tau_{\text{miati}}^s, \tau_{\text{mati}}^s]\}$. We emphasize again that $k_{pf} \equiv 0$, $k_{cf} \equiv 0$ and $e_f \equiv 0$ in $\mathcal{H}_5$.
Similar to $\mathcal{H}_5$, $\mathcal{H}_6$ is a specialized model of $\mathcal{H}_1$, with lower dimension. The functions will be used to define $\mathcal{H}_6$ and $\mathcal{H}_6^y$ have the same form as $\mathcal{H}_1$, but all the elements related to $e_s$, $k_{ps}$ and $k_{cs}$ are removed.
We define $y \coloneqq z - \overline{H}(x)$, where $\overline{H}$ comes from SA\ref{assum:standing-ss}. Let $\xi_6^y \coloneqq (x,y,e_f,\tau_f, \kappa_f) \in \mathbb{X}_6$
Then $\mathcal{H}_6^y$, which is $\mathcal{H}_6$ after changing the coordinates, is given by 
\begin{equation*}
    \mathcal{H}_6^y:\left\{
\begin{aligned}
    \dot{\xi}_6^y &= F_6^y(\xi_6^y, \epsilon),\ \xi_6^y \in \mathcal{C}_6^{y,\epsilon}, \\
    {\xi_6^y}^+ &= G_{6,f}(\xi_6^y), \ \xi_6^y\in \mathcal{D}_{6,f}^{y,\epsilon},
\end{aligned}
    \right.
\end{equation*}
where  $F_6^y(\xi_6^y) \coloneqq \big(f_x(x,y+\overline{H}(x),e_f), \tfrac{1}{\epsilon} F_f^y(x,y,e_f,\epsilon) \big)$,
with $F_f^y$ coming from system \eqref{eqn: H_2^y}, $C_6^{y,\epsilon} \coloneqq \{ \xi_6^y \in \mathbb{X}_6 |\epsilon \tau_f \in [0, \tau_{\text{mati}}^f]\}$ , $G_{6,f}^y(\xi_6^y) \coloneqq \big(x, y,h_f(\kappa_f, e_f), 0, \kappa_f + 1\big)$ and $D_{6,f}^{y,\epsilon} \coloneqq \{ \xi_6^y \in \mathbb{X}_6^y | \epsilon \tau_f \in [\tau_{\text{miati}}^f, \tau_{\text{mati}}^f]\}$.


We recall that $\xi_f\coloneqq (y,e_f, \tau_f, \kappa_f)$, and we can derive a hybrid boundary-layer system $\mathcal{H}_{6,bl}$ by first writing $\tau_{\text{mati}}^f =  \epsilon T^*$ and $\tau_{\text{miati}}^f = a \epsilon T^*$, then we have
\begin{equation*}
    \mathcal{H}_{6,bl}:\left\{
\begin{aligned}
    (\tfrac{\partial x}{\partial \sigma}, \tfrac{\partial \xi_f}{\partial \sigma}) &= \big(0, F_f^y(x,y,e_f,0) \big),\ \xi_6^y \in \mathcal{C}_6^{y,0}, \\
    {\xi_6^y}^+ &= \big(x,h_f(\kappa_f, e_f), 0, \kappa_f + 1\big), \ \xi_6^y\in \mathcal{D}_{6,f}^{y,0},
\end{aligned}
    \right.    
\end{equation*}
where $\mathcal{C}_6^{y,0}\coloneqq \{\xi_6^y \in \mathbb{X} | \tau_f \in [0, T^*] \}$ and $\mathcal{D}_{6,f}^{y,0} \coloneqq \{\xi_6^y \in \mathbb{X} | \tau_f \in [aT^*, T^*] \}$.


Then we can derive a continuous time reduced system $\mathcal{H}_{6,r}$ given by 
\begin{equation*}
    \mathcal{H}_{6,r} : \begin{cases}
        \tfrac{\partial x}{\partial \sigma} = f_z(x,\overline{H}(x),0).
    \end{cases}
\end{equation*}



Since $\mathcal{H}_{6,bl}$ has the same form as $\mathcal{H}_{bl}$, Assumption \ref{Assumption boundary layer system} is applicable to $\mathcal{H}_{6,bl}$, then by Lemma \ref{Lemma MATI}, there exist $U_f(x, \xi_f)$ that satisfies \eqref{eqn: Uf}, with $\mathcal{C}_{2,bl}^{y,0}$ and $\mathcal{D}_f^{y,0}$ replaced by $\mathcal{C}_6^{y,0}$ and $\mathcal{D}_{6,f}^{y,0}$, respectively. But since there are no slow transmissions, Assumption \ref{Assumption reduced model} and \eqref{eqn: Us} in Lemma \ref{Lemma MATI} should be combined and replaced by the following assumption.
\begin{assum}
    Consider $\mathcal{H}_6^y$, there exist locally Lipschitz function $V_s(x)$, class $\mathcal{K}_\infty$ functions $\underline{\alpha}_{V_s}$ and $\overline{\alpha}_{V_s}$, positive real number $a_s$ and positive definite function $\psi_s$ such that for all $x \in \mathbb{R}^{n_x}$, we have
    \begin{align}
    \underline{\alpha}_{V_s}\left(\left| x \right|\right)\leq {V_s}(x) & \leq \overline{\alpha}_{V_s}\left(\left| x\right|\right) \\
     \left< \tfrac{\partial {V_s}(x)}{\partial x},f_x(x,\overline{H}(x),0)  \right> &\leq -a_s \psi_s^2 \left(| x |\right).
     \label{eqn: Assumption stable slow subsystem, Us flow}
    \end{align}
    \label{Assumption Stable slow subsystem}
\end{assum}

Moreover, Assumption \ref{Assumption interconnection} is applicable to $\mathcal{H}_6^y$, where $\xi_s$, $F_s^y(x,y,e_s,e_f)$ and $F_s^y(x,0,e_s,0)$ reduced to $x$, $f_x(x,y+\overline{H}(x),e_f)$ and $f_x(x,\overline{H}(x),0)$, respectively.



We define the set the set $\mathcal{E}_6 \coloneqq \{\xi_6 \in \mathbb{X}_6 | x=0 \wedge z = 0 \wedge e_f=0 \}$.
\begin{cor}
    Consider system $\mathcal{H}_6$ and suppose Assumptions \ref{Assumption reduced model}, \ref{Assumption Extra 2} and \ref{Assumption Stable slow subsystem} hold, and Assumption \ref{Assumption interconnection} holds with $\widetilde{\mathcal{C}} = \mathcal{C}_6^{y,\epsilon}$.
    Let $b_1$, $b_2$, and $b_3$ come from Assumption \ref{Assumption interconnection}, $a_s$ comes from Assumption \ref{Assumption Stable slow subsystem} and $a_f$ comes from Lemma \ref{Lemma MATI}. Then for any $\tau_{\text{miati}}^f \leq \tau_{\text{mati}}^f \leq T(L_f, \gamma_f, \lambda_f^*)$, the following statement holds:

    There exists a $\mathcal{KL}$-function $\beta$, such that for all $\Delta,\nu>0$, there exists $\epsilon^* >0$ such that for all $0<\epsilon<\epsilon^*$, any solution $\xi_6$ with $ |\xi_6(0,0)|_{\mathcal{E}_6}<\Delta$ satisfies $|\xi_6(t,j)|_{\mathcal{E}_6} \leq \beta(|\xi_6(0,0)|_{\mathcal{E}_6}, t+j) + \nu$ for any $(t,j)\in \text{dom} \, \xi_6$.
    
    \label{Corollary Stable slow subsystem}
\end{cor}
\textbf{Proof:}
    Corollary \ref{Corollary Stable slow subsystem} can be proved using similar steps as Theorem \ref{Theorem H_1} and Corollary \ref{Corollary Stable fast subsystem}, except the composite Lyapunov function is now $U(x,\xi_f) = V_s(x) + dU_f(\xi_f) $ and is non-increasing at slow transmissions.


==> Chapters/7_Stable_subsystem.tex <==
% This section will study two specific configurations of our single-channel SPNCSs, both of them are special cases of $\mathcal{H}_1$, with lower dimension.

This section will study two typical configurations usually adopted in the literature, which is assuming either slow or fast subsystems are stable, and thus need not be stabilized via the network. In this paper, we do not need these assumptions, but these are special cases of our main results.


\subsection{Stable fast subsystem}
The first scenario is when the plant $\mathcal{P}$ has a stable fast subsystem (i.e., boundary layer system) and the controller is designed to stabilise the slow subsystem. This scenario typically arises when we have sensors or actuators operating on a faster time scale.
%
Subsequently, the plant only needs to transmit slow output $y_s$ and the controller only has slow control input $u_s$. The plant and controller below are in the form of \eqref{eqn:plant} and \eqref{eqn:controller}, where $k_{pf}$ and $k_{cf}$ are removed.
\begin{equation*}
    \mathcal{P}\!:\!
    \begin{cases}
    \dot x_p \!\!\!\!\!\!&= f_p(x_p, z_p,\hat u)\\
    \epsilon \dot z_p\!\!\!\!\!\! &= g_p(x_p, z_p, \hat u) \\
    y_p \!\!\!\!\!\!&= y_s = k_{p_s}(x_p)  , 
    \end{cases} \qquad
    \mathcal{C}\!:\!
    \begin{cases}
    \dot x_c \!\!\!\!\!\!&= f_c(x_c, z_c, \hat{y}_p)\\
    \epsilon \dot z_c \!\!\!\!\!\!&= g_c(x_c, z_c, \hat y_p) \\
    u \!\!\!\!\!\!&= u_s = k_{c_s}(x_c).
    \end{cases}
\end{equation*}

Given the exclusive presence of slow transmissions within the communication channel, a simpler version of clock mechanism \eqref{eqn: Stefan timer} is used to govern the system dynamics:
\begin{equation*}
    \tau_{\text{miati}}^s \leq t_{k+1}^s - t_k^s \leq \tau_{\text{mati}}^s, \ \forall t_k^s, t_{k+1}^s\in \mathcal{T}^s, k \in \mathbb{Z}_{\geq 0}.
\end{equation*}
Moreover, the networked induced error becomes $e_s =  (\hat{y}_s - y_s, \hat{u}_s - u_s)$, and $e_f$ no longer exist. We define the state $\xi_5 \coloneqq (x,e_s, \tau_s, \kappa_s, z)\in \mathbb{X}_5$, with $\mathbb{X}_5\coloneqq \mathbb{R}^{n_x}\times \mathbb{R}^{n_{e_s}}\times  \mathbb{R}_{\geq 0} \times \mathbb{Z}_{\geq 0} \times \mathbb{R}^{n_z}$, and we define our system by the hybrid model $\mathcal{H}_5$, and we omit its expression here.

% \begin{equation*}
%     \mathcal{H}_5:\left\{
% \begin{aligned}
%     \dot{\xi}_5 &= F_5(\xi_5),\ \xi_5 \in \mathcal{C}_5, \\
%     \xi^+ &= G_{5,s}(\xi_5), \ \xi_5 \in \mathcal{D}_{5,s},
% \end{aligned}
%     \right.
% \end{equation*}
% where $F_5(\xi_5) \coloneqq \big(f_x(x,z,e_s,e_f), f_{e_s}(x,z,e_s,e_f),1,0,$ $\tfrac{1}{\epsilon} g_z(x,z,e_s,e_f) \big)$, $C_5 \coloneqq \{ \xi_5 \in \mathbb{X}_5 | \tau_s \in [0, \tau_{\text{mati}}^s]\}$ , $G_{5,s}(\xi_5) \coloneqq (x, h_s(\kappa_s, e_s), 0, \kappa_s + 1, z)$ and $D_{5,s} \coloneqq \{ \xi_5 \in \mathbb{X}_5 | \tau_s \in [\tau_{\text{miati}}^s, \tau_{\text{mati}}^s]\}$. We emphasize again that $k_{pf} \equiv 0$, $k_{cf} \equiv 0$ and $e_f \equiv 0$ in $\mathcal{H}_5$.

We again define $y \coloneqq z - \overline{H}(x,e_s)$, where $\overline{H}$ comes from SA\ref{assum:standing-ss}. Let $\xi_5^y \coloneqq (x,e_s,\tau_s, \kappa_s,y) \in \mathbb{X}_5$,
then we can define $\mathcal{H}_5^y$, which is $\mathcal{H}_5$ after changing the coordinate. \cyan{Since $\mathcal{H}_5$ is a special case of $\mathcal{H}_1$, the functions we used to define $\mathcal{H}_5^y$ have the same form as $\mathcal{H}_2^y$ (e.g., \eqref{eq:functions}), but no longer depend on the state $e_f$, nor functions $k_{pf}$ and $k_{cf}$. For example, we will have that $\dot x$ equals to $f_x\big(x,y+\overline{H}(x,e_s), e_s\big)$, not $f_x\big(x,y+\overline{H}(x,e_s), e_s, e_f\big)$.} Then we can write
\begin{equation*}
    \mathcal{H}_5^y:\left\{
\begin{aligned}
    \dot{\xi}_5^y &= F_5^y(\xi_5^y, \epsilon),\ \xi_5^y \in \mathcal{C}_5^y, \\
    {\xi_5^y}^+ &= G_{5,s}(\xi_5^y), \ \xi_5^y \in \mathcal{D}_{5,s}^y,
\end{aligned}
    \right.
\end{equation*}
where $F_5^y(\xi_5^y, \epsilon) \coloneqq \big(F_s^y(x,y,e_s), \tfrac{1}{\epsilon} (\epsilon \tfrac{\partial y}{\partial t})  \big)$, with $F_s^y$ and $\epsilon \tfrac{\partial y}{\partial t}$ come from system \eqref{eqn: H_2^y}, $C_5^y \coloneqq \{ \xi_5^y \in \mathbb{X}_5 | \tau_s \in [0, \tau_{\text{mati}}^s]\}$, $G_{5,s}^y(\xi_5^y) \coloneqq \big(x, h_s(\kappa_s, e_s), 0, \kappa_s + 1, h_y(x,e_s,y)\big)$ and $D_{5,s}^y \coloneqq \{ \xi_5^y \in \mathbb{X}_5^y | \tau_s \in [\tau_{\text{miati}}^s, \tau_{\text{mati}}^s]\}$.







Furthermore, we can derive a continuous time boundary-layer system $\mathcal{H}_{5,bl}$
\begin{equation*}
    \mathcal{H}_{5,bl} : \begin{cases}
        \tfrac{\partial y}{\partial \sigma} = g_z(x,y+\overline{H}(x,e_s),e_s),
    \end{cases}
\end{equation*}
and a NCS $\mathcal{H}_{5,r}$ 
\begin{equation*}
    \mathcal{H}_{5,r}:\left\{
\begin{aligned}
    \dot{\xi_s} &= F_s^y(\xi_s),\ \xi_5^y \in \mathcal{C}_5^y, \\
    \xi_s^+ &= \big(x,h_s(\kappa_s, e_s), 0, \kappa_s + 1\big), \ \xi_5^y\in \mathcal{D}_{5,s}^y,
\end{aligned}
    \right.    
\end{equation*}
where we recall that $\xi_s \coloneqq (x,e_s,\tau_s, \kappa_s)$.

\cyan{We note that only $\mathcal{H}_{5,r}$ is a NCS, while $\mathcal{H}_{5,bl}$ is not, as it is already stable and does not need to be stabilized through network transmissions. Consequently, we need to modify relevant assumptions. In this case, we adjust Assumption \ref{Assumption boundary layer system}, resulting in Assumption \ref{Assumption Stable fast subsystem} below. 
}

%Assumptions \ref{Assumption reduced model}-\ref{Assumption interconnection} are written for a more general model (i.e., $\mathcal{H}_2^y$), when we apply them to a specialized model with lower dimension, we ignore the states that does not exist in the specialized model. \cyan{For instance, $\mathcal{H}_5$ does not have the state $e_f$, then when we apply Assumption \ref{Assumption reduced model} to it, $f_x(x, \overline{H}(x,e_s),e_s,0)$ is replaced by $f_x(x, \overline{H}(x,e_s),e_s)$.} At the same time, Lemma \ref{Lemma MATI} is applicable to any reduced and boundary layer system with the same form as $\mathcal{H}_r$ and $\mathcal{H}_{bl}$, and if only Assumption \ref{Assumption reduced model} or \ref{Assumption boundary layer system} holds, we can conclude \eqref{eqn: Us} or \eqref{eqn: Uf}, respectively.
 %
%Since $\mathcal{H}_{5,r}$ has the same form as $\mathcal{H}_r$, Assumption \ref{Assumption reduced model} is applicable to $\mathcal{H}_{5,r}$, then by Lemma \ref{Lemma MATI}, there exist $U_s$ satisfies inequalities in \eqref{eqn: Us} with $\mathcal{C}_{2,r}^{y,0}$ and $\mathcal{D}_{2,r}^{y,0}$ replaced by $\mathcal{C}_5^y$ and $\mathcal{D}_{5,s}^y$, respectively. Since there is no fast transmissions, Assumption \ref{Assumption boundary layer system} and \eqref{eqn: Uf} in Lemma \ref{Lemma MATI} should be combined and replaced by the following assumption.




\begin{assum}
    Consider $\mathcal{H}_5^y$, there exist locally Lipschitz function $V_f(x,y)$, class $\mathcal{K}_\infty$ functions $\underline{\alpha}_{V_f}$ and $\overline{\alpha}_{V_f}$, positive real number $a_f$ and positive definite function $\psi_f$ such that for all $\xi_5 \in \mathbb{X}_5$, we have
    \begin{align}
    \underline{\alpha}_{V_f}\left(\left| y \right|\right)\leq {V_f}(x,y) & \leq \overline{\alpha}_{V_f}\left(\left| y\right|\right) \\
     \left< \tfrac{\partial {V_f}(x,y)}{\partial y},g_z(x,y+ \overline{H}(x, e_s),e_s)  \right> &\leq -a_f \psi_f^2 \left(| y |\right).
     \label{eqn: Assumption stable fast subsystem, Uf flow}
    \end{align}
    \label{Assumption Stable fast subsystem}
\end{assum}
We define the set $\mathcal{E}_5 \coloneqq \{\xi_5 \in \mathbb{X}_5 | x=0 \wedge e_s = 0 \wedge z=0 \}$.
\begin{cor}
    Consider system $\mathcal{H}_5$ and suppose Assumptions \ref{Assumption reduced model}, \ref{Assumption Vf at slow transmission}, \ref{Assumption Extra 2} and \ref{Assumption Stable fast subsystem} hold, and Assumption \ref{Assumption interconnection} holds with $\widetilde{\mathcal{C}} =  \mathcal{C}_5^y$.
    Let $b_1$, $b_2$, and $b_3$ come from Assumption \ref{Assumption interconnection}, $a_s$ comes from Lemma \ref{Lemma MATI} and $a_f$ comes from Assumption \ref{Assumption Stable fast subsystem}. Then for any $\tau_{\text{miati}}^s \leq \tau_{\text{mati}}^s \leq T(L_s, \gamma_s, \lambda_s^*)$, the following statement holds:

    There exists a $\mathcal{KL}$-function $\beta$, such that for all $\Delta, \nu>0$, there exist $\epsilon^* >0$ such that for all $0<\epsilon<\epsilon^*$, any solution $\xi_5$ with $ |\xi_5(0,0)|_{\mathcal{E}_5}<\Delta$ satisfies $|\xi_5(t,j)|_{\mathcal{E}_5} \leq \beta(|\xi_5(0,0)|_{\mathcal{E}_5}, t+j) + \nu$ for any $(t,j)\in \text{dom} \, \xi_5$.
    \label{Corollary Stable fast subsystem}
\end{cor}
\textbf{Proof:} The proof of Corollary \ref{Corollary Stable fast subsystem} is in the Appendix. 


















\subsection{Stable slow subsystem}
The second scenario is when the plant has a stable slow subsystem. A controller is designed to stabilise the fast subsystem.
Subsequently, the plant only needs to transmit fast output $y_f$ and the controller only has fast control input $u_f$. 
The plant and controller shown below are in the form of \eqref{eqn:plant} and \eqref{eqn:controller}, where $k_{ps} $ and $k_{cs}$ are removed.
\begin{equation*}
    \mathcal{P}\!:\!
    \begin{cases}
    \dot x_p \!\!\!\!\!\!&= f_p(x_p, z_p,\hat u)\\
    \epsilon \dot z_p\!\!\!\!\!\! &= g_p(x_p, z_p, \hat u) \\
    y_p \!\!\!\!\!\!&= y_f = k_{p_f}(x_p,z_p)  , 
    \end{cases} \;
    \mathcal{C}\!:\!
    \begin{cases}
    \dot x_c \!\!\!\!\!\!&= f_c(x_c, z_c, \hat{y}_p)\\
    \epsilon \dot z_c \!\!\!\!\!\!&= g_c(x_c, z_c, \hat y_p) \\
    u \!\!\!\!\!\!&= u_f = k_{c_f}(x_c,z_c) ,
    \end{cases}
\end{equation*}

Given the exclusive presence of fast transmissions within the communication channel, a simpler version of clock mechanism \eqref{eqn: Stefan timer} is used to govern the system dynamics as follows:
\begin{equation*}
    \tau_{\text{miati}}^f \leq t_{k+1}^f - t_k^f \leq \tau_{\text{mati}}^f, \ \forall t_k^f, t_{k+1}^f\in \mathcal{T}^f, k \in \mathbb{Z}_{\geq 0},
\end{equation*}
where $\tau_{\text{miati}}^f \geq \tau_{\text{miati}}^f$. Moreover, the networked induced error is $e_f =  (\hat{y}_f - y_f, \hat{u}_f - u_f)$ and $e_s$ does not exist. By define the state $\xi_6 \coloneqq (x,z,e_f, \tau_f, \kappa_f,)\in \mathbb{X}_6$, where $\mathbb{X}_6\coloneqq \mathbb{R}^{n_x} \times \mathbb{R}^{n_z} \times \mathbb{R}^{n_{e_f}}\times  \mathbb{R}_{\geq 0} \times \mathbb{Z}_{\geq 1} $, we can define our system by the hybrid model $\mathcal{H}_6$, which we skip its expression here.


% \begin{equation*}
%     \mathcal{H}_5:\left\{
% \begin{aligned}
%     \dot{\xi}_5 &= F_5(\xi_5),\ \xi_5 \in \mathcal{C}_5, \\
%     \xi^+ &= G_{5,s}(\xi_5), \ \xi_5 \in \mathcal{D}_{5,s},
% \end{aligned}
%     \right.
% \end{equation*}
% where $F_5(\xi_5) \coloneqq \big(f_x(x,z,e_s,e_f), f_{e_s}(x,z,e_s,e_f),1,0,$ $\tfrac{1}{\epsilon} g_z(x,z,e_s,e_f) \big)$, $C_5 \coloneqq \{ \xi_5 \in \mathbb{X}_5 | \tau_s \in [0, \tau_{\text{mati}}^s]\}$ , $G_{5,s}(\xi_5) \coloneqq (x, h_s(\kappa_s, e_s), 0, \kappa_s + 1, z)$ and $D_{5,s} \coloneqq \{ \xi_5 \in \mathbb{X}_5 | \tau_s \in [\tau_{\text{miati}}^s, \tau_{\text{mati}}^s]\}$. We emphasize again that $k_{pf} \equiv 0$, $k_{cf} \equiv 0$ and $e_f \equiv 0$ in $\mathcal{H}_5$.
Similar to $\mathcal{H}_5$, $\mathcal{H}_6$ is a specialized model of $\mathcal{H}_1$, with lower dimension. The functions will be used to define $\mathcal{H}_6$ and $\mathcal{H}_6^y$ have the same form as $\mathcal{H}_1$, but all the elements related to $e_s$, $k_{ps}$ and $k_{cs}$ are removed.
We define $y \coloneqq z - \overline{H}(x)$, where $\overline{H}$ comes from SA\ref{assum:standing-ss}. Let $\xi_6^y \coloneqq (x,y,e_f,\tau_f, \kappa_f) \in \mathbb{X}_6$
Then $\mathcal{H}_6^y$, which is $\mathcal{H}_6$ after changing the coordinates, is given by 
\begin{equation*}
    \mathcal{H}_6^y:\left\{
\begin{aligned}
    \dot{\xi}_6^y &= F_6^y(\xi_6^y, \epsilon),\ \xi_6^y \in \mathcal{C}_6^{y,\epsilon}, \\
    {\xi_6^y}^+ &= G_{6,f}(\xi_6^y), \ \xi_6^y\in \mathcal{D}_{6,f}^{y,\epsilon},
\end{aligned}
    \right.
\end{equation*}
where  $F_6^y(\xi_6^y) \coloneqq \big(f_x(x,y+\overline{H}(x),e_f), \tfrac{1}{\epsilon} F_f^y(x,y,e_f,\epsilon) \big)$,
with $F_f^y$ coming from system \eqref{eqn: H_2^y}, $C_6^{y,\epsilon} \coloneqq \{ \xi_6^y \in \mathbb{X}_6 |\epsilon \tau_f \in [0, \tau_{\text{mati}}^f]\}$ , $G_{6,f}^y(\xi_6^y) \coloneqq \big(x, y,h_f(\kappa_f, e_f), 0, \kappa_f + 1\big)$ and $D_{6,f}^{y,\epsilon} \coloneqq \{ \xi_6^y \in \mathbb{X}_6^y | \epsilon \tau_f \in [\tau_{\text{miati}}^f, \tau_{\text{mati}}^f]\}$.


We recall that $\xi_f\coloneqq (y,e_f, \tau_f, \kappa_f)$, and we can derive a hybrid boundary-layer system $\mathcal{H}_{6,bl}$ by first writing $\tau_{\text{mati}}^f =  \epsilon T^*$ and $\tau_{\text{miati}}^f = a \epsilon T^*$, then we have
\begin{equation*}
    \mathcal{H}_{6,bl}:\left\{
\begin{aligned}
    (\tfrac{\partial x}{\partial \sigma}, \tfrac{\partial \xi_f}{\partial \sigma}) &= \big(0, F_f^y(x,y,e_f,0) \big),\ \xi_6^y \in \mathcal{C}_6^{y,0}, \\
    {\xi_6^y}^+ &= \big(x,h_f(\kappa_f, e_f), 0, \kappa_f + 1\big), \ \xi_6^y\in \mathcal{D}_{6,f}^{y,0},
\end{aligned}
    \right.    
\end{equation*}
where $\mathcal{C}_6^{y,0}\coloneqq \{\xi_6^y \in \mathbb{X} | \tau_f \in [0, T^*] \}$ and $\mathcal{D}_{6,f}^{y,0} \coloneqq \{\xi_6^y \in \mathbb{X} | \tau_f \in [aT^*, T^*] \}$.


Then we can derive a continuous time reduced system $\mathcal{H}_{6,r}$ given by 
\begin{equation*}
    \mathcal{H}_{6,r} : \begin{cases}
        \tfrac{\partial x}{\partial \sigma} = f_z(x,\overline{H}(x),0).
    \end{cases}
\end{equation*}



Since $\mathcal{H}_{6,bl}$ has the same form as $\mathcal{H}_{bl}$, Assumption \ref{Assumption boundary layer system} is applicable to $\mathcal{H}_{6,bl}$, then by Lemma \ref{Lemma MATI}, there exist $U_f(x, \xi_f)$ that satisfies \eqref{eqn: Uf}, with $\mathcal{C}_{2,bl}^{y,0}$ and $\mathcal{D}_f^{y,0}$ replaced by $\mathcal{C}_6^{y,0}$ and $\mathcal{D}_{6,f}^{y,0}$, respectively. But since there are no slow transmissions, Assumption \ref{Assumption reduced model} and \eqref{eqn: Us} in Lemma \ref{Lemma MATI} should be combined and replaced by the following assumption.
\begin{assum}
    Consider $\mathcal{H}_6^y$, there exist locally Lipschitz function $V_s(x)$, class $\mathcal{K}_\infty$ functions $\underline{\alpha}_{V_s}$ and $\overline{\alpha}_{V_s}$, positive real number $a_s$ and positive definite function $\psi_s$ such that for all $x \in \mathbb{R}^{n_x}$, we have
    \begin{align}
    \underline{\alpha}_{V_s}\left(\left| x \right|\right)\leq {V_s}(x) & \leq \overline{\alpha}_{V_s}\left(\left| x\right|\right) \\
     \left< \tfrac{\partial {V_s}(x)}{\partial x},f_x(x,\overline{H}(x),0)  \right> &\leq -a_s \psi_s^2 \left(| x |\right).
     \label{eqn: Assumption stable slow subsystem, Us flow}
    \end{align}
    \label{Assumption Stable slow subsystem}
\end{assum}

Moreover, Assumption \ref{Assumption interconnection} is applicable to $\mathcal{H}_6^y$, where $\xi_s$, $F_s^y(x,y,e_s,e_f)$ and $F_s^y(x,0,e_s,0)$ reduced to $x$, $f_x(x,y+\overline{H}(x),e_f)$ and $f_x(x,\overline{H}(x),0)$, respectively.



We define the set the set $\mathcal{E}_6 \coloneqq \{\xi_6 \in \mathbb{X}_6 | x=0 \wedge z = 0 \wedge e_f=0 \}$.
\begin{cor}
    Consider system $\mathcal{H}_6$ and suppose Assumptions \ref{Assumption reduced model}, \ref{Assumption Extra 2} and \ref{Assumption Stable slow subsystem} hold, and Assumption \ref{Assumption interconnection} holds with $\widetilde{\mathcal{C}} = \mathcal{C}_6^{y,\epsilon}$.
    Let $b_1$, $b_2$, and $b_3$ come from Assumption \ref{Assumption interconnection}, $a_s$ comes from Assumption \ref{Assumption Stable slow subsystem} and $a_f$ comes from Lemma \ref{Lemma MATI}. Then for any $\tau_{\text{miati}}^f \leq \tau_{\text{mati}}^f \leq T(L_f, \gamma_f, \lambda_f^*)$, the following statement holds:

    There exists a $\mathcal{KL}$-function $\beta$, such that for all $\Delta,\nu>0$, there exists $\epsilon^* >0$ such that for all $0<\epsilon<\epsilon^*$, any solution $\xi_6$ with $ |\xi_6(0,0)|_{\mathcal{E}_6}<\Delta$ satisfies $|\xi_6(t,j)|_{\mathcal{E}_6} \leq \beta(|\xi_6(0,0)|_{\mathcal{E}_6}, t+j) + \nu$ for any $(t,j)\in \text{dom} \, \xi_6$.
    
    \label{Corollary Stable slow subsystem}
\end{cor}
\textbf{Proof:}
    Corollary \ref{Corollary Stable slow subsystem} can be proved using similar steps as Theorem \ref{Theorem H_1} and Corollary \ref{Corollary Stable fast subsystem}, except the composite Lyapunov function is now $U(x,\xi_f) = V_s(x) + dU_f(\xi_f) $ and is non-increasing at slow transmissions.
% \begin{cor}
%     Consider system $\mathcal{H}_6$ and suppose Assumptions \ref{Assumption reduced model}, \ref{Assumption Stable slow subsystem} hold, and Assumption \ref{Assumption interconnection} hold for almost all $\xi_6^y \in \mathcal{C}_6^{y,\epsilon}$.
%     Let $b_1$, $b_2$, and $b_3$ come from Assumption \ref{Assumption interconnection}, $a_s$ come from Assumption \ref{Assumption Stable slow subsystem} and $a_f$ come from Lemma \ref{Lemma MATI}. Then there exist $\epsilon^* >0$ such that for all $0<\epsilon<\epsilon^*$, $\tau_{\text{mati}}^f \leq T(L_f, \gamma_f, \lambda_f^*)$, the following statement holds:

%     There exists a $\mathcal{KL}$-function $\beta$, such that for all $\Delta,\nu > 0$, any solution $\xi_6$ with $ |\xi_6(0,0)|_{\mathcal{E}_6}<\Delta$ satisfies $|\xi_6(t,j)|_{\mathcal{E}_6} \leq \beta(|\xi_6(0,0)|_{\mathcal{E}_6}, t+j) + \nu$ for any $(t,j)\in \text{dom} \, \xi_6$.
    
%     \label{Corollary Stable slow subsystem}
% \end{cor}
% \begin{proof}
%     The proof of Corollary \ref{Corollary Stable slow subsystem} is in the Appendix.
% \end{proof}


==> Chapters/Test_shorted_Introduction.tex <==
Networked control systems (NCSs) integrate feedback control loops with real-time communication networks \cite{definition}. The rapid evolution of network technologies has expanded NCS applications across various sectors, such as industrial automation, smart transportation, telemedicine, and exploration \cite{xu2018survey}, often involving processes on multiple time scales. For instance, robotic systems have rapid control loops for electrical dynamics and slower ones for mechanical dynamics. Most state-of-the-art research in NCSs \cite{dragan_stability,carnevale_stability,heijmans2017computing} typically overlook this multi-scale structure, leading to designs demanding high data transmission rates to maintain system stability or robustness. This is especially problematic for Internet of Things (IoT) devices, which are generally wireless, battery-powered, and have limited bandwidth, processing power, and storage capacity. Extending singularly perturbed methods \cite{nonlinear_systems_Khalil} to NCSs results in singularly perturbed NCSs (SPNCSs).

SPNCSs have gained substantial attention for their applicability in various engineering disciplines. Researchers have developed various control and analysis techniques for both linear and nonlinear SPNCSs. For instance, \cite{wang2021observer,song2019dynamic,cheng2021ultimate,lei2022event} introduced a range of control and analysis techniques for linear SPNCSs. For nonlinear SPNCSs, \cite{Romain_ETC} formulated stabilizing event-triggered feedback laws based on the reduced model, assuming stable fast dynamics, while \cite{SPNCS} established sufficient conditions for stability in time-triggered, two-time-scale nonlinear SPNCSs under the scenario of separate channels for slow and fast signals, which is not always practical.

In this paper, we consider a two-time scale nonlinear system stabilized by a dynamical output feedback controller, inspired by both linear \cite{linear1980,linear2018,linear2010} and nonlinear \cite{output_feedback} research on dynamic controllers for singularly perturbed dynamical systems (SPSs) without network constraints. Unlike previous work \cite{SPNCS} that only transmits plant states, we address scenarios where both plant output and controller input are transmitted via a single communication channel, presenting challenges in allocating access for slow and fast signals. Our objective is to design a resource-efficient mechanism using dual clocks to manage the transmission of slow and fast signals, thereby stabilizing the SPNCS over a single communication channel.

We model the SPNCS as a hybrid SPS, with jump sets designed to satisfy the dual clock mechanism. Our hybrid SPS is more general compared to those in the literature \cite{sanfelice2011singular,wang2012analysis,6161309}, as its flow and jump sets depend on the time scale separation parameter, $\epsilon$. Following an emulation-based approach, we demonstrate that the stability properties of the SPNCS, such as semi-global practical asymptotic stability, can be ensured by sufficiently fast transmission of both slow and fast variables. Specifically, we use a Lyapunov-based analysis to determine the maximum allowable transmission interval (MATI) for the slow and fast dynamics.

Compared to our preliminary work \cite{Single_channel_NCS_CDC}, we relax a restrictive condition on the minimum allowable transmission interval (MIATI) and present conditions guaranteeing stronger stability properties, such as uniformly globally asymptotic stability (UGAS) and uniformly globally exponential stability (UGES). While many literature results \cite{Romain_ETC} assume that either the slow or fast subsystem is stable without control, our methodology does not rely on this assumption. Our framework accommodates scenarios involving stable slow or fast subsystems as special cases.

Our results are novel even for linear time-invariant (LTI) systems. Compared to linear works \cite{song2019dynamic,lei2022event} that assumed the sampled-data structure, we consider SPNCSs with scheduling protocols. While \cite{wang2021observer,song2019dynamic,cheng2021ultimate,lei2022event} assumed periodic transmissions, we allow aperiodic transmissions and consider inter-event continuous behavior, often ignored by others. We recast several assumptions as linear matrix inequalities (LMIs) and demonstrate that other assumptions can always be satisfied. Finally, we illustrate the benefits of our approach through a numerical case study.





%%%%%%%%%%%%%
\textbf{Notation:} The sets of real numbers and integers larger than or equal to an integer $n$ are denoted by $\mathbb{R}_{\geq n}$ and $\mathbb{Z}_{\geq n}$, respectively. 
%
% A function $\alpha: \mathbb{R}_{\geq 0} \rightarrow \mathbb{R}_{\geq 0}$ is said to be of class $\mathcal{K}$ if it is continuous, positive definite and strictly increasing. It is of class $\mathcal{K}_{\infty}$ if it is also unbounded. 
% %
% A function $\beta:\mathbb{R}_{\geq 0} \times \mathbb{R}_{\geq 0} \rightarrow \mathbb{R}_{\geq 0}$ is said to be class $\mathcal{KL}$ if for each $s \geq 0$, the function $\beta(s, \cdot)$ is decreasing to zero in the second argument and for each constant $t \geq 0$, the function $\beta(\cdot, t)$ is of class $\mathcal{K}$.
%
For vectors $v_i\in \mathbb{R}^n$, $i\in \{1,2,\cdots, N\}$, we denote the vector $[v_1^\top \; v_2^\top \; \cdots \; v_N^\top]^\top$ by $(v_1, v_2, \cdots, v_N)$, and inner product by $\left< \cdot , \cdot \right>$. 
%
Given a vector $x\in \mathbb{R}^{n_x}$ and a non-empty closed set $\mathcal{A} \subseteq \mathbb{R}^{n_x}$, the distance from $x$ to $\mathcal{A}$ is denoted by $|x|_\mathcal{A} \coloneqq \min_{y\in \mathcal{A}}|x-y|$.
We use $U^\circ(x;v)$ to denote the Clarke generalized derivative \cite[Eqn. (20)]{teel2000assigning} of a locally Lipschitz function $U$ at $x$ in the direction of $v$. 
%
For a real symmetric matrix $P$, we denote its maximum and minimum eigenvalues by $\lambda_{\text{max}}(P)$ and $\lambda_{\text{min}}(P)$ respectively. The logic AND operator is denoted by $\wedge$.


